Clifford algebra and the projective model of homogeneous metric spaces: Foundations

This paper is to serve as a key to the projective (homogeneous) model developed by Charles Gunn (arXiv:1101.4542 [math.MG]). The goal is to explain the underlying concepts in a simple language and give plenty of examples. It is targeted to physicists and engineers and the emphasis is on explanation rather than rigorous proof. The projective model is based on projective geometry and Clifford algebra. It supplements and enhances vector and matrix algebras. It also subsumes complex numbers and quaternions. Projective geometry augmented with Clifford algebra provides a unified algebraic framework for describing points, lines, planes, etc, and their transformations, such as rotations, reflections, projections, and translations. The model is relevant not only to Euclidean space but to a variety of homogeneous metric spaces.

==> g-100+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-100+0_0.pdf}%
}%


==> g-100.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-100+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294246147,3Droll=0,3Droo=410.407255607294246147,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-100+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-100+0.prc}}


==> g-101+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-101+0_0.pdf}%
}%


==> g-101.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-101+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-101+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-101+0.prc}}


==> g-102+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-102+0_0.pdf}%
}%


==> g-102.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-102+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-102+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-102+0.prc}}


==> g-103+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-103+0_0.pdf}%
}%


==> g-103.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-103+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-103+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-103+0.prc}}


==> g-104+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-104+0_0.pdf}%
}%


==> g-104.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-104+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-104+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-104+0.prc}}


==> g-105+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-105+0_0.pdf}%
}%


==> g-105.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-105+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-105+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-105+0.prc}}


==> g-106+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-106+0_0.pdf}%
}%


==> g-106.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-106+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -409.971468858114008071,3Droll=0,3Droo=409.971468858114008071,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-106+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-106+0.prc}}


==> g-107+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-107+0_0.pdf}%
}%


==> g-107.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-107+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858114121758,3Droll=0,3Droo=409.971468858114121758,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-107+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-107+0.prc}}


==> g-108+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-108+0_0.pdf}%
}%


==> g-108.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-108+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858114064915,3Droll=0,3Droo=409.971468858114064915,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-108+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-108+0.prc}}


==> g-109+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-109+0_0.pdf}%
}%


==> g-109.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-109+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-109+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-109+0.prc}}


==> g-110+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-110+0_0.pdf}%
}%


==> g-110.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 237.279750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,118.639875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-110+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -409.971468858114008071,3Droll=0,3Droo=409.971468858114008071,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-110+0.js]{254.9525pt}{234.8775pt}{\ASYprefix\jobname-110+0.prc}}


==> g-111+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-111+0_0.pdf}%
}%


==> g-111.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-111+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -439.7966203249255841,3Droll=0,3Droo=439.7966203249255841,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-111+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-111+0.prc}}


==> g-112+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-112+0_0.pdf}%
}%


==> g-112.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-112+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -439.7966203249255841,3Droll=0,3Droo=439.7966203249255841,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-112+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-112+0.prc}}


==> g-113+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-113+0_0.pdf}%
}%


==> g-113.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-113+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858114178602,3Droll=0,3Droo=409.971468858114178602,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-113+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-113+0.prc}}


==> g-114+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-114+0_0.pdf}%
}%


==> g-114.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-114+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-114+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-114+0.prc}}


==> g-115+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-115+0_0.pdf}%
}%


==> g-115.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-115+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-115+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-115+0.prc}}


==> g-116+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-116+0_0.pdf}%
}%


==> g-116.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-116+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -409.971468858114008071,3Droll=0,3Droo=409.971468858114008071,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-116+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-116+0.prc}}


==> g-117+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-117+0_0.pdf}%
}%


==> g-117.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-117+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -439.7966203249255841,3Droll=0,3Droo=439.7966203249255841,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-117+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-117+0.prc}}


==> g-118+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-118+0_0.pdf}%
}%


==> g-118.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-118+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -439.796620324925697787,3Droll=0,3Droo=439.796620324925697787,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-118+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-118+0.prc}}


==> g-119+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-119+0_0.pdf}%
}%


==> g-119.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-119+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-119+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-119+0.prc}}


==> g-120+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-120+0_0.pdf}%
}%


==> g-120.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-120+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -439.796620324925697787,3Droll=0,3Droo=439.796620324925697787,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-120+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-120+0.prc}}


==> g-121+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-121+0_0.pdf}%
}%


==> g-121.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 224.231000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.115500)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-121+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -397.358738818155870831,3Droll=0,3Droo=397.358738818155870831,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-121+0.js]{254.9525pt}{221.82875pt}{\ASYprefix\jobname-121+0.prc}}


==> g-122+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-122+0_0.pdf}%
}%


==> g-122.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 231.257250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,115.628625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-122+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-122+0.js]{254.9525pt}{228.855pt}{\ASYprefix\jobname-122+0.prc}}


==> g-123+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-123+0_0.pdf}%
}%


==> g-123.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-123+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-123+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-123+0.prc}}


==> g-124+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-124+0_0.pdf}%
}%


==> g-124.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 237.279750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,118.639875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-124+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -409.971468858114008071,3Droll=0,3Droo=409.971468858114008071,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-124+0.js]{254.9525pt}{234.8775pt}{\ASYprefix\jobname-124+0.prc}}


==> g-125+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-125+0_0.pdf}%
}%


==> g-125.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 221.219750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,110.609875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-125+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -399.96653321195077524,3Droll=0,3Droo=399.96653321195077524,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-125+0.js]{254.9525pt}{218.8175pt}{\ASYprefix\jobname-125+0.prc}}


==> g-126+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-126+0_0.pdf}%
}%


==> g-126.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-126+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -406.944060929735371701,3Droll=0,3Droo=406.944060929735371701,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-126+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-126+0.prc}}


==> g-127+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-127+0_0.pdf}%
}%


==> g-127.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-127+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -418.149930769026411781,3Droll=0,3Droo=418.149930769026411781,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-127+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-127+0.prc}}


==> g-128+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-128+0_0.pdf}%
}%


==> g-128.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-128+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -427.803668427023751519,3Droll=0,3Droo=427.803668427023751519,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-128+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-128+0.prc}}


==> g-129+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-129+0_0.pdf}%
}%


==> g-129.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 223.227250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,111.613625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-129+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -582.488012149737755863,3Droll=0,3Droo=582.488012149737755863,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-129+0.js]{254.9525pt}{220.825pt}{\ASYprefix\jobname-129+0.prc}}


==> g-130+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-130+0_0.pdf}%
}%


==> g-130.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 237.279750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,118.639875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-130+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -399.000038011455501419,3Droll=0,3Droo=399.000038011455501419,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-130+0.js]{254.9525pt}{234.8775pt}{\ASYprefix\jobname-130+0.prc}}


==> g-131+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-131+0_0.pdf}%
}%


==> g-131.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 231.257250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,115.628625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-131+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.499894470580898087,3Droll=0,3Droo=410.499894470580898087,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-131+0.js]{254.9525pt}{228.855pt}{\ASYprefix\jobname-131+0.prc}}


==> g-132+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-132+0_0.pdf}%
}%


==> g-132.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 231.257250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,115.628625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-132+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858114178602,3Droll=0,3Droo=409.971468858114178602,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-132+0.js]{254.9525pt}{228.855pt}{\ASYprefix\jobname-132+0.prc}}


==> g-133+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-133+0_0.pdf}%
}%


==> g-133.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 232.261000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,116.130500)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-133+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -438.895625811763352431,3Droll=0,3Droo=438.895625811763352431,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-133+0.js]{254.9525pt}{229.85875pt}{\ASYprefix\jobname-133+0.prc}}


==> g-134+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-134+0_0.pdf}%
}%


==> g-134.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 213.189750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,106.594875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-134+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -398.019261270355741544,3Droll=0,3Droo=398.019261270355741544,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-134+0.js]{254.9525pt}{210.7875pt}{\ASYprefix\jobname-134+0.prc}}


==> g-135+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-135+0_0.pdf}%
}%


==> g-135.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-135+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -418.826747676222225891,3Droll=0,3Droo=418.826747676222225891,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-135+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-135+0.prc}}


==> g-136+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-136+0_0.pdf}%
}%


==> g-136.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 238.283510pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,119.141755)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-136+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -408.432816112569923916,3Droll=0,3Droo=408.432816112569923916,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-136+0.js]{254.9525pt}{235.88125pt}{\ASYprefix\jobname-136+0.prc}}


==> g-137+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-137+0_0.pdf}%
}%


==> g-137.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 229.249750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,114.624875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-137+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.845712903221851775,3Droll=0,3Droo=411.845712903221851775,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-137+0.js]{254.9525pt}{226.8475pt}{\ASYprefix\jobname-137+0.prc}}


==> g-138+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-138+0_0.pdf}%
}%


==> g-138.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-138+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -417.770080012105609057,3Droll=0,3Droo=417.770080012105609057,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-138+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-138+0.prc}}


==> g-139.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-139_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887807,113.958449)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.107512,229.676408)(-1.000000,-0.500000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,221.199366)(0.000000,-0.500000){$\mathbb{T}^1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-101.028989,153.355495)(-0.800000,0.250000){$J(\textbf{a})$}


==> g-140.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-140_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-3.848402,113.958449)(-0.500000,-1.000000){$d$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.107512,229.676408)(-1.000000,-0.500000){$a$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,221.199366)(0.000000,-0.500000){$\mathbb{T}^{1*}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-150.404558,136.356972)(-0.500000,0.000000){$\textbf{a}$}


==> g-41+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-41+0_0.pdf}%
}%


==> g-41.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-41+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751624274,3Droll=0,3Droo=410.889700647751624274,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-41+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-41+0.prc}}


==> g-42+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-42+0_0.pdf}%
}%


==> g-42.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 234.268510pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,117.134255)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-42+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -458.244188366010234859,3Droll=0,3Droo=458.244188366010234859,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-42+0.js]{254.9525pt}{231.86625pt}{\ASYprefix\jobname-42+0.prc}}


==> g-43+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-43+0_0.pdf}%
}%


==> g-43.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 210.178500pt{}%
\kern 299.512250pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-149.756125,105.089250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-43+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -500.547393955850793645,3Droll=0,3Droo=500.547393955850793645,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-43+0.js]{297.11pt}{207.77625pt}{\ASYprefix\jobname-43+0.prc}}


==> g-44+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-44+0_0.pdf}%
}%


==> g-44.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-44+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.952455161797274741,3Droll=0,3Droo=411.952455161797274741,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-44+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-44+0.prc}}


==> g-45+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-45+0_0.pdf}%
}%


==> g-45.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 217.204750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,108.602375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-45+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.8897006477513969,3Droll=0,3Droo=410.8897006477513969,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-45+0.js]{254.9525pt}{214.8025pt}{\ASYprefix\jobname-45+0.prc}}


==> g-46+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-46+0_0.pdf}%
}%


==> g-46.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 212.186000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,106.093000)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-46+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -406.882962558835401978,3Droll=0,3Droo=406.882962558835401978,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-46+0.js]{254.9525pt}{209.78375pt}{\ASYprefix\jobname-46+0.prc}}


==> g-47+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-47+0_0.pdf}%
}%


==> g-47.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 202.148500pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,101.074250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-47+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.491592795065855626,3Droll=0,3Droo=410.491592795065855626,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-47+0.js]{254.9525pt}{199.74625pt}{\ASYprefix\jobname-47+0.prc}}


==> g-48+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-48+0_0.pdf}%
}%


==> g-48.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 201.144750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,100.572375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-48+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751737961,3Droll=0,3Droo=410.889700647751737961,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-48+0.js]{254.9525pt}{198.7425pt}{\ASYprefix\jobname-48+0.prc}}


==> g-49.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-49_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887807,57.051837)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-62.451837,116.114121)(-1.000000,-0.500000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-31.418075,57.051837)(-0.500000,-1.000000){$\textbf{e}^0$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-57.051837,88.085598)(0.000000,-0.500000){$\textbf{e}^1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-89.994787,43.675768)(-1.000000,-0.874375){$-1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-29.508887,75.827906)(0.000000,0.125625){$+1$}


==> g-50.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-50_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887807,57.051837)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-62.451837,116.114121)(-1.000000,-0.500000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-31.418075,57.051837)(-0.500000,-1.000000){$\textbf{e}^0$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-57.051837,88.085598)(0.000000,-0.500000){$\textbf{e}^1$}


==> g-51+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-51+0_0.pdf}%
}%


==> g-51.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 202.148500pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,101.074250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-51+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.952455161797388428,3Droll=0,3Droo=411.952455161797388428,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-51+0.js]{254.9525pt}{199.74625pt}{\ASYprefix\jobname-51+0.prc}}


==> g-52+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-52+0_0.pdf}%
}%


==> g-52.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 202.148500pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,101.074250)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-52+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -411.952455161797104211,3Droll=0,3Droo=411.952455161797104211,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-52+0.js]{254.9525pt}{199.74625pt}{\ASYprefix\jobname-52+0.prc}}


==> g-53+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-53+0_0.pdf}%
}%


==> g-53.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-53+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751737961,3Droll=0,3Droo=410.889700647751737961,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-53+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-53+0.prc}}


==> g-54+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-54+0_0.pdf}%
}%


==> g-54.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-54+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.952455161797274741,3Droll=0,3Droo=411.952455161797274741,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-54+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-54+0.prc}}


==> g-55+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-55+0_0.pdf}%
}%


==> g-55.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-55+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -410.889700647751453744,3Droll=0,3Droo=410.889700647751453744,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-55+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-55+0.prc}}


==> g-56+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-56+0_0.pdf}%
}%


==> g-56.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-56+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.952455161797274741,3Droll=0,3Droo=411.952455161797274741,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-56+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-56+0.prc}}


==> g-57+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-57+0_0.pdf}%
}%


==> g-57.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-57+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751624274,3Droll=0,3Droo=410.889700647751624274,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-57+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-57+0.prc}}


==> g-58+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-58+0_0.pdf}%
}%


==> g-58.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-58+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.952455161797388428,3Droll=0,3Droo=411.952455161797388428,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-58+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-58+0.prc}}


==> g-59+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-59+0_0.pdf}%
}%


==> g-59.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-59+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -410.889700647751453744,3Droll=0,3Droo=410.889700647751453744,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-59+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-59+0.prc}}


==> g-60+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-60+0_0.pdf}%
}%


==> g-60.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-60+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -411.952455161797104211,3Droll=0,3Droo=411.952455161797104211,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-60+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-60+0.prc}}


==> g-61+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-61+0_0.pdf}%
}%


==> g-61.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-61+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -410.889700647751453744,3Droll=0,3Droo=410.889700647751453744,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-61+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-61+0.prc}}


==> g-62+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-62+0_0.pdf}%
}%


==> g-62.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-62+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -411.952455161797331584,3Droll=0,3Droo=411.952455161797331584,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-62+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-62+0.prc}}


==> g-63+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-63+0_0.pdf}%
}%


==> g-63.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-63+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751737961,3Droll=0,3Droo=410.889700647751737961,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-63+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-63+0.prc}}


==> g-64+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-64+0_0.pdf}%
}%


==> g-64.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-64+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -411.952455161797331584,3Droll=0,3Droo=411.952455161797331584,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-64+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-64+0.prc}}


==> g-65.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-65_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-50.928431,48.020774)(0.000000,-0.250000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-175.855157,87.057678)(-1.000000,-0.583337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-160.451839,204.246840)(-0.750000,0.000000){$\textbf{aI}$}


==> g-66.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-66_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-50.928431,48.020774)(0.000000,-0.250000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-153.141811,98.414351)(-1.000000,-0.583337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-198.490807,28.140709)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-24.739594,123.046627)(-0.750000,0.000000){$\textbf{a}\cdot\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-71.230145,23.103452)(-0.500000,-0.750000){$\textbf{e}_0\wedge(\textbf{a}\cdot\textbf{P})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-151.522284,67.272307)(-0.250000,0.250000){0.894427 0.447214 -0.447214 0.894427}{$|\textbf{a}\vee\textbf{P}|$}


==> g-67.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-67_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-99.119917,141.707441)(0.000000,-1.000000){\textbf{P}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-56.532392,170.099124)(0.000000,-0.779180){\textbf{Q}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-25.029808,199.914309)(-0.833333,0.220820){$\textbf{P}\vee\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-95.503367,84.926631)(-0.166667,-0.750000){$\textbf{e}_0\wedge(\textbf{P}\vee\textbf{Q})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-189.882581,129.354989)(-1.000000,-0.612513){$\textbf{P}\times\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-93.456157,162.282386)(-0.166667,0.000000){0.832050 0.554700 -0.554700 0.832050}{$\norm{\textbf{P}\vee\textbf{Q}}$}


==> g-68.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-68_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-99.119917,141.707441)(0.000000,-1.000000){\textbf{P}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-39.447993,133.338091)(-0.166667,-1.000000){\textbf{N}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-48.310988,184.393522)(-0.833333,0.000000){$\textbf{P}\vee\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-104.967261,99.122473)(-0.166667,-0.750000){$\textbf{e}_0\wedge(\textbf{P}\vee\textbf{N})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-175.686740,138.818883)(-1.000000,-0.714430){$\textbf{P}\times\textbf{N}$}


==> g-69.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-69_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-89.782690,177.937496)(-0.500000,-0.862071){$\textbf{N}_1=\textbf{a}\wedge\textbf{b}_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-139.797720,185.292901)(-1.000000,-0.750000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-77.490918,136.239798)(0.000000,-0.083337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-214.751763,164.850890)(-1.000000,-0.612071){$\textbf{b}_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-148.045911,103.662301)(-0.500000,0.137929){$\textbf{e}_0\wedge\textbf{b}_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-175.469966,157.755195)(-0.250000,0.250000){0.894427 0.447214 -0.447214 0.894427}{$|\textbf{e}_{12}\vee\textbf{N}_1|$}


==> g-70.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-70_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-38.677661,194.694169)(-0.500000,0.137929){$\textbf{N}_2=\textbf{a}\wedge\textbf{b}_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-145.618015,196.933491)(-1.000000,-0.750000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-77.490918,136.239798)(0.000000,-0.083337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-147.744070,42.910271)(0.000000,-0.112071){$\textbf{b}_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-198.834497,72.868008)(-0.500000,-0.862071){$\textbf{e}_0\wedge\textbf{b}_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalignT(-172.930536,152.676336)(-0.250000,0.250000){0.894427 0.447214 -0.447214 0.894427}{$|\textbf{e}_{12}\vee\textbf{N}_2|$}


==> g-71.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-71_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-97.735996,145.048521)(0.000000,-0.360630){$\textbf{P}_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-50.928431,48.020774)(0.000000,-0.250000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-130.270243,131.143898)(-1.000000,-0.583337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-60.079159,191.248735)(-1.000000,0.137929){$\textbf{b}_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-79.685045,124.972569)(0.000000,-0.362071){$\textbf{e}_0\wedge\textbf{b}_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-105.619434,125.565303)(-0.580515,-0.794874){$\alpha_1$}


==> g-72.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-72_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-97.735996,145.048521)(0.000000,-0.360630){$\textbf{P}_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-50.928431,48.020774)(0.000000,-0.250000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-130.270243,131.143898)(-1.000000,-0.583337){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-187.430358,56.260783)(0.000000,-0.862071){$\textbf{b}_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-125.236948,165.124472)(-1.000000,-0.362071){$\textbf{e}_0\wedge\textbf{b}_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-121.978554,147.777708)(-1.000000,-0.294874){$\alpha_2$}


==> g-73.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-73_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-44.402795,23.532118)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-140.323521,59.873472)(0.000000,-0.500000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-72.183482,93.943491)(0.000000,-0.273640){$(\textbf{P}\cdot\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-190.614382,85.425987)(0.000000,-0.273640){$(\textbf{P}\wedge\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-204.531887,173.440204)(-1.000000,-0.500000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-196.153550,159.383531)(-0.500000,-0.773640){$(\textbf{N}\cdot\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-164.922699,194.594798)(-0.500000,0.226360){$(\textbf{N}\wedge\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-99.760996,186.500378)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-56.748726,59.661364)(0.000000,-0.023640){$(\textbf{a}\cdot\textbf{b})\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-45.605821,170.457417)(-0.250000,-0.773640){$(\textbf{a}\wedge\textbf{b})\textbf{b}^{-1}$}


==> g-74.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-74_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-125.886925,186.500378)(-1.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-140.323521,66.960972)(-0.166667,0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-194.021384,163.219198)(0.000000,-0.273640){$(\textbf{a}\cdot\textbf{P})\textbf{P}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-170.099124,56.532392)(0.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-140.323521,59.873472)(0.000000,-0.273640){$(\textbf{Q}\cdot\textbf{P})\textbf{P}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-201.831887,62.573472)(-0.500000,0.226360){$(\textbf{Q}\times\textbf{P})\textbf{P}^{-1}$}


==> g-75.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-75_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-74.715376,95.284846)(0.000000,0.000000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-21.622929,25.441306)(0.000000,0.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-78.988020,66.566963)(-1.000000,-0.902231){$-\textbf{b}\textbf{a}\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-177.706207,200.050156)(0.000000,0.000000){$\textbf{c}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-200.050156,177.706207)(-1.000000,-1.000000){$\textbf{b}\textbf{c}\textbf{b}^{-1}$}


==> g-76.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-76_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-21.622929,25.441306)(0.000000,0.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-61.080949,204.246840)(-0.750000,0.000000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-88.265155,176.140204)(-0.500000,0.000000){$\textbf{b}\textbf{N}\textbf{b}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-141.707441,84.924075)(0.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.924075,141.707441)(0.000000,-0.814617){$\textbf{b}\textbf{Q}\textbf{b}^{-1}$}


==> g-77.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-77_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-151.308608,154.278608)(-0.450000,0.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-141.707441,84.924075)(0.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-206.513724,95.646992)(0.000000,-0.314617){$\textbf{Q}\textbf{b}\textbf{Q}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-61.080949,204.246840)(-0.750000,0.000000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-58.665995,128.437726)(-0.250000,-0.814617){$\textbf{Q}\textbf{N}\textbf{Q}^{-1}$}


==> g-78.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-78_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.924075,113.315758)(0.000000,-1.000000){$\textbf{R}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-141.707441,84.924075)(0.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-30.300539,140.323521)(-0.375000,-0.814617){$\textbf{R}\textbf{Q}\textbf{R}^{-1}$}


==> g-79.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-79_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-188.409566,184.591190)(-1.000000,-1.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-111.931838,145.048521)(0.000000,-0.279180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-162.506616,209.781558)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.485155,178.165204)(-0.100000,0.250000){$\mathsf{proj}(\textbf{Q};\textbf{b})+3\mathsf{rej}(\textbf{Q};\textbf{b})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-100.101697,209.781558)(0.000000,-0.250000){$\mathsf{proj}(\textbf{a};\textbf{b})+3\mathsf{rej}(\textbf{a};\textbf{b})$}


==> g-80.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-80_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-111.931838,173.440204)(0.000000,-0.500000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.997917,141.707441)(-1.000000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-139.969200,172.531670)(-1.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.997917,84.924075)(-1.000000,-0.750000){$\mathsf{proj}(\textbf{Q};\textbf{P})+3\mathsf{rej}(\textbf{Q};\textbf{P})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-131.920158,105.016248)(-1.000000,-0.250000){$\mathsf{proj}(\textbf{a};\textbf{P})+3\mathsf{rej}(\textbf{a};\textbf{P})$}


==> g-81.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-81_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-28.140709,113.315758)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.924075,113.315758)(0.000000,-1.000000){$\textbf{R}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-43.388252,156.808741)(0.000000,-0.500000){$R\textbf{P}\!R^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-163.219198,176.140204)(-0.500000,0.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-145.312900,142.612900)(-1.000000,-0.500000){$R\textbf{b}R^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-145.048521,62.573472)(-0.500000,0.000000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-167.824472,51.557740)(-1.000000,-0.500000){$R\textbf{N}R^{-1}$}


==> g-82.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-82_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-125.886925,186.500378)(-1.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-28.140709,113.315758)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-170.442814,46.878935)(-0.500000,0.166663){$\textbf{e}_0\wedge\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-168.474449,186.500378)(-1.000000,-0.500000){$T\textbf{b}T^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-83.540155,145.048521)(0.000000,-0.500000){$T\textbf{P}T^{-1}$}


==> g-83.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-83_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-56.532392,155.903283)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-39.287841,24.739594)(0.000000,-0.250000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\ASYalign(-25.142087,180.634977)(-0.750000,0.000000){$\textbf{a}\cdot\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-208.927743,178.651539)(-0.333333,0.250000){$\mathsf{f}(\textbf{a})$}


==> g-84.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-84_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-56.532392,155.903283)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-205.172966,198.490807)(-1.000000,-1.000000){$\textbf{A}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-155.487521,106.217838)(-1.000000,-0.750000){$\mathsf{f}(\textbf{A})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-61.782660,90.174343)(-1.000000,-0.000000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-90.965155,59.873472)(-1.000000,-0.250000){$\mathsf{f}(\textbf{N})$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-61.782660,29.572601)(-1.000000,-0.881097){$\textbf{N}\times\textbf{P}$}


==> g-85+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-85+0_0.pdf}%
}%


==> g-85.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 220.216000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,110.108000)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-85+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -407.200825427707400195,3Droll=0,3Droo=407.200825427707400195,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-85+0.js]{254.9525pt}{217.81375pt}{\ASYprefix\jobname-85+0.prc}}


==> g-86+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-86+0_0.pdf}%
}%


==> g-86.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-86+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-86+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-86+0.prc}}


==> g-87+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-87+0_0.pdf}%
}%


==> g-87.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-87+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-87+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-87+0.prc}}


==> g-88+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-88+0_0.pdf}%
}%


==> g-88.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 229.249750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,114.624875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-88+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-88+0.js]{254.9525pt}{226.8475pt}{\ASYprefix\jobname-88+0.prc}}


==> g-89+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-89+0_0.pdf}%
}%


==> g-89.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-89+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-89+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-89+0.prc}}


==> g-90+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-90+0_0.pdf}%
}%


==> g-90.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 237.279750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,118.639875)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-90+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -405.655466983347139376,3Droll=0,3Droo=405.655466983347139376,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-90+0.js]{254.9525pt}{234.8775pt}{\ASYprefix\jobname-90+0.prc}}


==> g-91+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-91+0_0.pdf}%
}%


==> g-91.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-91+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -399.011094516032130741,3Droll=0,3Droo=399.011094516032130741,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-91+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-91+0.prc}}


==> g-92+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-92+0_0.pdf}%
}%


==> g-92.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-92+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -411.288960546472026181,3Droll=0,3Droo=411.288960546472026181,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-92+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-92+0.prc}}


==> g-93+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-93+0_0.pdf}%
}%


==> g-93.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-93+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-93+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-93+0.prc}}


==> g-94+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-94+0_0.pdf}%
}%


==> g-94.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-94+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-94+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-94+0.prc}}


==> g-95+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-95+0_0.pdf}%
}%


==> g-95.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-95+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-95+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-95+0.prc}}


==> g-96+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-96+0_0.pdf}%
}%


==> g-96.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-96+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-96+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-96+0.prc}}


==> g-97+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-97+0_0.pdf}%
}%


==> g-97.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-97+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-97+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-97+0.prc}}


==> g-98+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-98+0_0.pdf}%
}%


==> g-98.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-98+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.407255607294359834,3Droll=0,3Droo=410.407255607294359834,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-98+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-98+0.prc}}


==> g-99+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-99+0_0.pdf}%
}%


==> g-99.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-99+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-99+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-99+0.prc}}

